Transferable Unsupervised Outlier Detection Framework for Human Semantic Trajectories

Semantic trajectories, which enrich spatial-temporal data with textual information such as trip purposes or location activities, are key for identifying outlier behaviors critical to healthcare, social security, and urban planning. Traditional outlier detection relies on heuristic rules, which requires domain knowledge and limits its ability to identify unseen outliers. Besides, there lacks a comprehensive approach that can jointly consider multi-modal data across spatial, temporal, and textual dimensions. Addressing the need for a domain-agnostic model, we propose the Transferable Outlier Detection for Human Semantic Trajectories (TOD4Traj) framework.TOD4Traj first introduces a modality feature unification module to align diverse data feature representations, enabling the integration of multi-modal information and enhancing transferability across different datasets. A contrastive learning module is further pro-posed for identifying regular mobility patterns both temporally and across populations, allowing for a joint detection of outliers based on individual consistency and group majority patterns. Our experimental results have shown TOD4Traj's superior performance over existing models, demonstrating its effectiveness and adaptability in detecting human trajectory outliers across various datasets.

==> content/baselines.tex <==
We compare with several unsupervised trajectory outlier detection methods, including three rule-based non-deep learning methods and two state-of-the-art deep learning methods:\\
\textbf{OMPAD} \cite{basharat2008learning} is an outlier detection method that analyzes objects' movement patterns by counting the types of locations they visit. It identifies abnormal activities by measuring the deviations in moving trends compared to established normal patterns.\\
\textbf{MoNav-TT }\cite{zhang2012smarter} is an outlier detection algorithm tailored for urban human trajectory networks, where it detects outliers by measuring discrepancies in traffic distances. In particular, a user is identified as an outlier if the traveled distance significantly deviates from their previous behavior.\\
\textbf{TRAOD } \cite{lee2008trajectory} is a partition-and-detect
framework for trajectory outlier detection, which partitions a
trajectory into a set of line segments, and then, detects outlying
line segments for trajectory outliers.\\
\textbf{DSVDD} \cite{ruff2018deep} is a deep one-class classification based outlier detection method. We generalize it to handle the task of semantic trajectory outlier detection in a most intuitive way. We map the weekly trajectories of each user to a high dimensional sphere by a deep neural network encoder. Then the distance of trajectories from the sphere's surface is quantified as an outlier score.\\
\textbf{DAE} \cite{zhou2017anomaly,dotti2020hierarchical} is a widely-used outlier detection method that leverages a deep autoencoder. Utilizing an encoder-decoder model architecture, it reconstructs input trajectories, and the resulting reconstruction error is used as an outlier indicator, signifying deviations from the normal pattern.\\
\textbf{GM-VSAE} \cite{liu2020online} introduces a deep generative model called Gaussian Mixture Variational Sequence AutoEncoder (GM-VSAE) for anomalous trajectory detection. GM-VSAE excels in capturing complex sequential information within trajectories, representing different types of normal routes in a continuous latent space, and facilitating efficient anomaly detection.\\
\textbf{DeepTEA} \cite{han2022deeptea} is a recently proposed deep learning framework designed for time-dependent trajectory outlier detection by capturing the dynamics of traffic patterns and the temporal dependencies of movements. It uses a combination of convolutional neural networks (CNNs) and recurrent neural networks (RNNs) to learn the normal patterns of trajectories over time. This approach allows DeepTEA to effectively identify outliers by comparing new trajectory data against learned patterns, taking into account both spatial and temporal characteristics, thus providing accurate and efficient online detection of anomalous trajectories.

==> content/dataset.tex <==

The patterns of life simulation was designed to emulate human needs and behavior in an urban environment~\cite{zufle2023urban}. %Utilizing this simulation fosters the development of advanced research in the field of human behavior recognition.
Within the simulated environment, virtual entities referred to as agents perform actions that mirror human activities. These include attending work, forming friendships, engaging in social gatherings, and more. The agents' existence is crafted to resemble human life in a real-world environment (roads, buildings) obtained from OpenStreetMap~\cite{bennett2010openstreetmap}. Throughout their simulated lives, agents navigate to diverse locations, including restaurants, workplaces, residential apartments, and recreational venues.
A salient feature of the simulation is the generation of comprehensive log files. These logs contain extensive data regarding the agents, including their location and current state information, thus allowing for in-depth analysis and research.

In our study, we generated data by running simulations over four distinct maps, namely Fairfax County, Virginia, USA (FVA); the French Quarter of New Orleans, Louisiana, USA (NOLA); Atlanta, Georgia, USA (ATL); and Beijing, China (BJNG). The simulations were conducted over a period of 450 days to replicate normal life, followed by an additional 14 days to incorporate abnormal behavior into the regular patterns.
We introduced three specific types of abnormal behavior that define outliers trajectories:

\begin{itemize}
    \item \textbf{Hunger outlier:} An agent under this category becomes hungry more quickly. Such agents have to go to restaurants or their homes much more often.
    \item \textbf{Social outlier:} This type of agent randomly selects recreational sites to visit when needed, rather than being guided by their attributes and social network.%instead of using the agent's attributes and social network to guide their choice.
    \item \textbf{Work outlier:} Agents in this category abstain from going to work on workdays.
\end{itemize}

We further divided these abnormalities into three intensity levels: red, orange, and yellow. Red outliers exhibit extremely abnormal behavior, orange outliers act moderately abnormal, and yellow outliers display abnormal behavior less frequently. For example, a work outlier will decide not to go to work 100\%, 50\%, or 20\% of the time when classified as red, orange, or yellow, respectively. We divide the simulation into 450 simulation of days of normal behavior, followed by 14 days of a small number of agents exhibiting outlier behavior.Details are provided in Table~\ref{table:dataset}, and an extended version of the dataset can be found in \cite{amiri2024urban}.
%At the end of the normal period, we adjusted the behavior of a specific number of agents according to the types and levels of outliers described above, allowing us to analyze the effects of these abnormalities on the overall system.


\subsubsection{Real World Dataset}\label{app:geolife}


The real-world dataset for this study was created using the Microsoft Research Asia's GPS Trajectory dataset~\cite{zheng2010geolife}. Since the original data did not conform to a check-in format, we employed the method outlined in \cite{zheng2008mining} to extract stay points, thereby transforming the data to fit the check-in pattern used in life simulation studies.
Next, we utilized OpenStreetMap to categorize locations into four groups: apartments, workplaces, pubs, and restaurants. Given that OpenStreetMap encompasses a broad array of categories and types, we manually classified them into these four distinct groups.
Upon preprocessing the data, we eliminated agents with fewer than 50 records, resulting in a final count of 69 agents with a total of 14,080 training trajectories and 3,552 test trajectories. Within the context of the GeoLife dataset, we introduced a specific outlier type called the ``imposter outlier". An agent acting as an imposter outlier by switching the trajectories with another agent after a specific time point. %usurps the role of another user by replacing the normal user's ID with the outliers ID.
The dataset was then divided into two segments: 80\% of the stay points for training and introduced outliers into the remaining 20\% for test. %While a normal user appears to act as usual, the outlier exhibits the behavior of an entirely different person.



==> content/droped_content.tex <==
\begin{table*}[t]
    \centering
    \begin{adjustbox}{width=1.0\textwidth,center}
        \begin{tabular}{@{}lcccccccccccc@{}}
            \toprule
                                      & \multicolumn{4}{c}{ATL}     & \multicolumn{4}{c}{NOLA}        & \multicolumn{4}{c}{FVA}                                                                                                                                                      \\
            \cmidrule(lr){2-5} \cmidrule(l){6-9} \cmidrule(l){10-13}
            Model                     & Top-10 Hits                 & Top-100 Hits\textsuperscript{*} & AP score                 & AUC score       & Top-10 Hits & Top-100 Hits & AP score        & AUC score       & Top-10 Hits & Top-100 Hits & AP score        & AUC score       \\
            \midrule
            OMPAD                     & 0                           & 7                               & 0.0571                   & 0.5257          & 2           & 10           & 0.0776          & 0.5968          & 0           & 4            & 0.0598          & 0.5322          \\
            MoNav-TT                  & 1                           & 5                               & 0.0893                   & 0.4863          & 1           & 3            & 0.0503          & 0.5026          & 0           & 0            & 0.0501          & 0.5014          \\
            TRAOD                     & 1                           & 10                              & 0.0582                   & 0.5018          & 0           & 4            & 0.0485          & 0.5011          & 0           & 7            & 0.0515          & 0.5090          \\
            DSVDD\textsuperscript{**} & 5                           & 36                              & 0.2601                   & 0.5835          & 9           & 28           & 0.2093          & 0.5829          & 5           & 26           & 0.2166          & 0.5995          \\
            DAE\textsuperscript{**}   & 3                           & 17                              & 0.0962                   & 0.5465          & 1           & 7            & 0.0648          & 0.5885          & 1           & 7            & 0.0569          & 0.5138          \\
            GM-VSAE                   & 4                           & 29                              & 0.1987                   & 0.5564          & 5           & 20           & 0.1786          & 0.5672          & 4           & 22           & 0.1534          & 0.5859          \\
            DeepTEA                   & 5                           & 26                              & 0.2008                   & 0.6012          & 5           & 26           & 0.2186          & 0.6395          & 5           & 30           & 0.2221          & 0.6182          \\
            \midrule
            TOD4Traj-MLP              & \textbf{10}                 & 34                              & 0.2782                   & 0.6824          & \textbf{10} & 41           & 0.3376          & 0.6985          & \textbf{10} & 32           & 0.2509          & 0.6561          \\
            TOD4Traj-RNN              & \textbf{10}                 & 32                              & 0.2780                   & 0.6233          & \textbf{10} & 27           & 0.2325          & 0.5940          & \textbf{10} & 27           & 0.2325          & 0.5940          \\
            TOD4Traj-CNN              & \textbf{10}                 & \textbf{42}                     & \textbf{0.3205}          & \textbf{0.7215} & \textbf{10} & \textbf{46}  & \textbf{0.3631} & \textbf{0.7185} & \textbf{10} & \textbf{40}  & \textbf{0.3151} & \textbf{0.6669} \\
            TOD4Traj-Former           & \textbf{10}                 & 34                              & 0.2436                   & 0.6735          & \textbf{10} & 34           & 0.2903          & 0.6970          & \textbf{10} & 33           & 0.2171          & 0.6628          \\
            \midrule
                                      & \multicolumn{4}{c}{Geolife} & \multicolumn{4}{c}{ATL-Large}   & \multicolumn{4}{c}{BJNG}                                                                                                                                                     \\
            \cmidrule(lr){2-5} \cmidrule(l){6-9}\cmidrule(l){10-13}
            OMPAD                     & 1                           & 4                               & 0.1665                   & 0.1697          & 3           & 20           & 0.1461          & 0.6028          & 1           & 9            & 0.0704          & 0.5655          \\
            MoNav-TT                  & 0                           & 7                               & 0.2849                   & 0.3989          & 1           & 5            & 0.0893          & 0.4863          & 1           & 5            & 0.0893          & 0.4863          \\
            TRAOD                     & 4                           & 7                               & 0.1060                   & 0.5498          & 0           & 1            & 0.0030          & 0.4390          & 0           & 6            & 0.0553          & 0.5169          \\
            DSVDD\textsuperscript{**} & 7                           & 15                              & 0.6246                   & 0.7714          & 1           & 14           & 0.1010          & 0.4911          & 10          & 29           & 0.2155          & 0.5643          \\
            DAE\textsuperscript{**}   & 5                           & 12                              & 0.4627                   & 0.6234          & 4           & 19           & 0.1466          & 0.5641          & 0           & 10           & 0.0671          & 0.5568          \\
            GM-VSAE                   & 4                           & 13                              & 0.4892                   & 0.6034          & 2           & 12           & 0.1243          & 0.5482          & 4           & 16           & 0.1068          & 0.5479          \\
            DeepTEA                   & 6                           & 14                              & 0.5290                   & 0.7540          & 4           & 22           & 0.1752          & 0.6398          & 6           & 24           & 0.2084          & 0.5873          \\
            \midrule
            TOD4Traj-MLP              & \textbf{8}                  & \textbf{17}                     & \textbf{0.8512}          & \textbf{0.9397} & 4           & 28           & 0.2632          & 0.6737          & \textbf{10} & 34           & 0.2800          & 0.6587          \\
            TOD4Traj-RNN              & 7                           & 11                              & 0.6359                   & 0.7467          & 3           & 12           & 0.1310          & 0.5294          & \textbf{10} & 31           & 0.2573          & 0.6065          \\
            TOD4Traj-CNN              & 6                           & 16                              & 0.6756                   & 0.8542          & \textbf{10} & \textbf{40}  & \textbf{0.4572} & \textbf{0.7141} & \textbf{10} & \textbf{66}  & \textbf{0.4899} & \textbf{0.7513} \\
            TOD4Traj-Former           & 7                           & 16                              & 0.6283                   & 0.8889          & 8           & 27           & 0.2783          & 0.6852          & \textbf{10} & 33           & 0.2499          & 0.6219          \\
            \bottomrule
        \end{tabular}

    \end{adjustbox}
    \caption{Outlier detection performance for all datasets. The best performance for AP and AUC scores is highlighted for each dataset. \textsuperscript{*}We report Top-25 Hits instead of Top-100 for Geolife dataset due to its size constraint. \textsuperscript{**}For implementation of comparison methods DSVDD and DAE, we only report the best performance of deep learning based competitive methods among the choice of four deep encoders (MLP, RNN, CNN and Transformer) for each dataset due to the limitation of the space.}\label{table:performance}
    \vspace{-0.3cm}
\end{table*}
